Mutlitask Learning for Cross-Lingual Transfer of Semantic Dependencies

We describe a method for developing broad-coverage semantic dependency parsers for languages for which no semantically annotated resource is available. We leverage a multitask learning framework coupled with an annotation projection method. We transfer supervised semantic dependency parse annotations from a rich-resource language to a low-resource language through parallel data, and train a semantic parser on projected data. We make use of supervised syntactic parsing as an auxiliary task in a multitask learning framework, and show that with different multitask learning settings, we consistently improve over the single-task baseline. In the setting in which English is the source, and Czech is the target language, our best multitask model improves the labeled F1 score over the single-task baseline by 1.8 in the in-domain SemEval data (Oepen et al., 2015), as well as 2.5 in the out-of-domain test set. Moreover, we observe that syntactic and semantic dependency direction match is an important factor in improving the results.

==> TS_biLSTM_TS_FNN.tex <==
\begin{figure}[htbp]
    \centering
        \includegraphics[width=0.5\textwidth]{sdp_mtl_sep.pdf}
        \caption{MTL model with task-specific recurrent layer and FNNs.}
        \label{fig_sdp_mtl_sep}
\end{figure}

==> background.tex <==
\section{Background}


Broad-coverage semantic dependency parsing (SDP) \citep{oepen-etal-2014-semeval,oepen-etal-2015-semeval,che-etal-2016-semeval} aims to discover the underlying semantic relation existing between \emph {all} content words in the sentence. %%Maryam what about functional words?? --> 
In this semantic representation scheme, each word in the sentence might be the semantic argument of multiple predicates. Therefore, unlike dependency parsing that integrates labeled bi-lexical dependencies as a tree, SDP forms a directed acyclic graph over syntactic dependencies. %Furthermore, SDP provide a whole sentence semantic analysis, whereas typically SRL output is constrained by verbal or nominal predicates.
SDP yields a labeled directed graph whose vertices are tokens in the sentence. So in this sense, it is considered similar to dependency-based SRL. Contrary to SRL, however, where the main focus is on verbal and nominal predicates, SDP produces a semantic analysis for all words in the sentence. 

The SDP dataset introduced in the SemEval shared tasks \citep{oepen-etal-2014-semeval,oepen-etal-2015-semeval,che-etal-2016-semeval} consists of three main semantic formalisms, also known as target representations, slightly differ in the way they determine and label semantic relations. These representations are usually referred to as {\bf DM} (DELPH-IN minimal recursion), {\bf PSD} (Prague semantic dependencies) and {\bf PAS} (Enju predicate–argument structures). These formalisms consist of labeled directed graphs between content words in the sentence. In general, the node with an outgoing edge corresponds to the predicate, likewise, the node with an incoming edge shows the semantic argument. Analogously, edge labels are equivalent to the semantic roles in semantic role labeling. Each sentence has a unique {\tt top} node that shows the main predicate of the sentence. Figure \ref{fig_related_sdp} shows a sentence from SemEval 2015 data along with its bi-lexical semantic dependencies in DM, PAS and PSD representations. 

Besides differences in the way each semantic formalism determines and labels semantic relations,
the main difference between bi-lexical semantic dependencies in SDP and other semantic representation formalisms such as PropBank/FrameNet SRL and AMR lies in the range of semantic phenomena that are addressed in each model. Some semantic phenomena such as comparatives, possessives and various types of modification that convey the sentence meaning are not addressed/handled/targeted in the PropBank or AMR representations, while being extensively analyzed in the DM representation. Figure \ref{fig_srl_sdp} further demonstrates the difference between PropBank (SRL) and DM (SDP) bi-lexical semantic dependencies.



\input{fig/srl_sdp.tex}



==> fig/sdp_LF_UF.tex <==
\usepgfplotslibrary{groupplots}
\usetikzlibrary{patterns}

% \begin{figure*}[t!]
% \centering
% \scalebox{0.8}{
% \begin{tikzpicture}

% \pgfplotsset{small,samples=20,every tick label/.append style={font=\small}}
%     \begin{groupplot}[group style = {group size = 2 by 2, horizontal sep = 50pt}, width = 6.0cm, height = 5.0cm]
    
    
%     %%%%%%%%%%%%%% in-domain LF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \nextgroupplot[title ={in-domain},xtick={0.5,0.6,0.7,0.8,0.9,1},ylabel = Labeled F1, legend style = { column sep = 1pt, legend columns = 1, legend to name = grouplegend,legend cell align={left}},axis lines=left,
%     grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10}]
    
%             \addplot[
%                 color=blue,
%                 mark=star,
%                 dashed,
%                 thick
%                 ]
%                 coordinates {
%                 (0.5,56.51)(0.6,56.72)(0.7,57.07)(0.8,57.48)(0.9,56.94)
%                 };
%                 \addlegendentry{\scriptsize{Single}}%
            
%                 \addplot[
%                     color=red,
%                     mark=star,
%                     ]
%                     coordinates {
% 					(0.5,56.9)(0.6,57.35)(0.7,58.66)(0.8,58.32)(0.9,57.95)
%                     };
%                     \addlegendentry{\scriptsize{RNN+FNN}}

%                 \addplot[
%                     color=green,
%                     mark=triangle,
%                     ]
%                     coordinates {
% 					(0.5,56.93)(0.6,57.06)(0.7,57.46)(0.8,58.74)(0.9,58.68)
%                     };
%               \addlegendentry{\scriptsize{RNN+FNN+Task RNN}}
                    
%              \addplot[
%                     color=black,
%                     mark=o,
%                     ]
%                     coordinates {
% 						(0.5,56.96)(0.6,57.82)(0.7,58.66)(0.8,59.29)(0.9,57.52)
%                     };
%             \addlegendentry{\scriptsize{RNN}}
            
%             \addplot[
% 	            color=purple,
% 	            mark=square,
% 	            ]
% 	            coordinates {
% 	            (0.5,56.66)(0.6,57.47)(0.7,57.89)(0.8,57.68)(0.9,57.68)
% 	            };
%             \addlegendentry{\scriptsize{RNN+Task RNN}}
     
%     %%%%%%%%%%%%%% out-domain LF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \nextgroupplot[title = {out-of-domain},xtick={0.5,0.6,0.7,0.8,0.9},axis lines=left,
%     grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10}]
             
%             \addplot[
%                 color=blue,
% 				mark=star,
% 				dashed,
% 				thick,
% 				]
%                 coordinates {
% 				(0.5,58)(0.6,58.42)(0.7,58.75)(0.8,58.75)(0.9,58.93)
%                 };
                
%             \addplot[
%                 color=red,
%                 mark=star,
%                 ]
%                 coordinates {
% 				(0.5,59.4)(0.6,60.13)(0.7,60.56)(0.8,60.5)(0.9,60.33)
%                 };
                
%             \addplot[
%                 color=green,
%                 mark=triangle,
%                 ]
%                 coordinates {
% 				(0.5,59.46)(0.6,59.43)(0.7,60.39)(0.8,60.81)(0.9,60.95)
%                 }; 
            
%           \addplot[
%             color=black,
%             mark=o,
%             ]
%             coordinates {
%             (0.5,59.83)(0.6,60.13)(0.7,61.23)(0.8,61.24)(0.9,59.67)
%             }; 
            
%           \addplot[
%             color=purple,
%             mark=square,
%             ]
%             coordinates {
%             (0.5,59.04)(0.6,59.83)(0.7,59.83)(0.8,59.83)(0.9,59.93)	
%             };
            
%     %%%%%%%%%%%%%% in-domain UF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \nextgroupplot[xtick={0.5,0.6,0.7,0.8,0.9},ylabel = Unlabeled F1, xlabel = Density median, legend style = { column sep = 1pt, legend columns = 1, legend to name = grouplegend,legend cell align={left}},axis lines=left,
%      grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10}]
%      \addplot[
%      color=blue,
%      mark=star,
%      dashed,
%      thick
%      ]
%      coordinates {
%      	(0.5,73)(0.6,73.15)(0.7,74.35)(0.8,74.26)(0.9,74.82)
%      };
%      \addlegendentry{\scriptsize{Single}}%
     
%      \addplot[
%      color=red,
%      mark=star,
%      ]
%      coordinates {
%      	(0.5,74.05)(0.6,74.67)(0.7,75.38)(0.8,75.72)(0.9,75.53)
%      };
%      \addlegendentry{\scriptsize{RNN+FNN}}
     
%      \addplot[
%      color=green,
%      mark=triangle,
%      ]
%      coordinates {
%      	(0.5,74.11)(0.6,73.99)(0.7,74.69)(0.8,75.31)(0.9,75.82)
%      };
%      \addlegendentry{\scriptsize{RNN+FNN+Task RNN}}
     
%      \addplot[
%      color=black,
%      mark=o,
%      ]
%      coordinates {
%      	(0.5,74.25)(0.6,74.97)(0.7,76.18)(0.8,76.43)(0.9,75.51)
%      };
%      \addlegendentry{\scriptsize{RNN}}
     
%      \addplot[
%         color=purple,
% 	    mark=square,
%      ]
%      coordinates {
%      	(0.5,73.83)(0.6,74.82)(0.7,75.46)(0.8,75.46)(0.9,75.16)
%      };
%      \addlegendentry{\scriptsize{RNN+Task RNN}}
     
%     %%%%%%%%%%%%%% out-domain UF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      \nextgroupplot[xtick={0.5,0.6,0.7,0.8,0.9},axis lines=left,
%      grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10},xlabel = Density median]
     
%      \addplot[
%      color=blue,
%      mark=star,
%      dashed,
%      ]
%      coordinates {
%      	(0.5,74.06)(0.6,74.61)(0.7,75.63)(0.8,75.83)(0.9,76.39)
%      };
     
%      \addplot[
%      color=red,
%      mark=star,
%      ]
%      coordinates {
%      	(0.5,76.27)(0.6,76.55)(0.7,77.16)(0.8,77.9)(0.9,77.41)
%      };
     
%      \addplot[
%      color=green,
%      mark=triangle,
%      ]
%      coordinates {
%      	(0.5,75.68)(0.6,75.66)(0.7,76.98)(0.8,77.31)(0.9,77.77)
%      }; 
     
%      \addplot[
%      color=black,
%      mark=o,
%      ]
%      coordinates {
%      	(0.5,76.14)(0.6,76.5)(0.7,77.88)(0.8,78.15)(0.9,77.17)
%      }; 
     
%      \addplot[
%         color=purple,
% 	    mark=square,
%      ]
%      coordinates {
%      	(0.5,75.45)(0.6,76.48)(0.7,77.31)(0.8,77.31)(0.9,77.05)	
%      };  
                        
%     \end{groupplot}

%     \node at ($(group c2r1) + (4.5,-5cm)$) {\ref{grouplegend}}; 
% \end{tikzpicture}
% }
% \caption{Labeled (top row) and unlabeled (bottom row) F1 scores for different MTL architecture compared to the baseline (Single). Graphs on the left and right columns show in-domain and out-of-domain results on the SemEval Czech test set respectively.}\label{sdp_LF_UF}
% \end{figure*}



\usepgfplotslibrary{groupplots}
\usetikzlibrary{patterns}

\begin{figure}[t!]
\centering
\scalebox{.95}{
\begin{tikzpicture}

\pgfplotsset{small,samples=20,every tick label/.append style={font=\scriptsize}}
    \begin{groupplot}[group style = {group size = 1 by 2, horizontal sep = 50pt}, width = 6.0cm, height = 5.0cm]
    
    
    %%%%%%%%%%%%%% in-domain LF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[title ={\scriptsize in-domain},xtick={0.5,0.6,0.7,0.8,0.9,1},ylabel = {\scriptsize Labeled F1}, y label style={at={(0.1,0.5)}}, legend style = { column sep = 1pt, legend columns = 1, legend to name = grouplegend,legend cell align={left}},axis lines=left,
    grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10}]
    
            \addplot[
                color=blue,
                mark=star,
                dashed,
                thick
                ]
                coordinates {
                (0.5,56.51)(0.6,56.72)(0.7,57.07)(0.8,57.48)(0.9,56.94)
                };
                \addlegendentry{\scriptsize{Single}}%
            
                \addplot[
                    color=red,
                    mark=star,
                    ]
                    coordinates {
					(0.5,56.9)(0.6,57.35)(0.7,58.66)(0.8,58.32)(0.9,57.95)
                    };
                    \addlegendentry{\scriptsize{RF}}

                \addplot[
                    color=green,
                    mark=triangle,
                    ]
                    coordinates {
					(0.5,56.93)(0.6,57.06)(0.7,57.46)(0.8,58.74)(0.9,58.68)
                    };
              \addlegendentry{\scriptsize{RF+TR}}
                    
             \addplot[
                    color=black,
                    mark=o,
                    ]
                    coordinates {
						(0.5,56.96)(0.6,57.82)(0.7,58.66)(0.8,59.29)(0.9,57.52)
                    };
            \addlegendentry{\scriptsize{R}}
            
            \addplot[
	            color=purple,
	            mark=square,
	            ]
	            coordinates {
	            (0.5,56.66)(0.6,57.47)(0.7,57.89)(0.8,57.68)(0.9,57.68)
	            };
            \addlegendentry{\scriptsize{R+TR}}
   
%%%%%%%%%%%%%% out-domain LF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[title = {\scriptsize out-of-domain}, xtick={0.5,0.6,0.7,0.8,0.9},axis lines=left,ylabel = {\scriptsize Labeled F1}, y label style={at={(0.1,0.5)}},
    grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10}]
             
            \addplot[
                color=blue,
				mark=star,
				dashed,
				thick,
				]
                coordinates {
				(0.5,58)(0.6,58.42)(0.7,58.75)(0.8,58.75)(0.9,58.93)
                };
                
            \addplot[
                color=red,
                mark=star,
                ]
                coordinates {
				(0.5,59.4)(0.6,60.13)(0.7,60.56)(0.8,60.5)(0.9,60.33)
                };
                
            \addplot[
                color=green,
                mark=triangle,
                ]
                coordinates {
				(0.5,59.46)(0.6,59.43)(0.7,60.39)(0.8,60.81)(0.9,60.95)
                }; 
            
          \addplot[
            color=black,
            mark=o,
            ]
            coordinates {
            (0.5,59.83)(0.6,60.13)(0.7,61.23)(0.8,61.24)(0.9,59.67)
            }; 
            
          \addplot[
            color=purple,
            mark=square,
            ]
            coordinates {
            (0.5,59.04)(0.6,59.83)(0.7,59.83)(0.8,59.83)(0.9,59.93)	
            };
            
                        
     \end{groupplot}

    \node at ($(6.0,-3.8cm)$) {\ref{grouplegend}}; 
\end{tikzpicture}
}
\caption{Labeled F1 scores for different multitask architectures compared to the single-task model in in-domain and out-of-domain SemEval Czech test set~\protect\cite{oepen-etal-2015-semeval}. \emph{TR} shows a setting for which there is task-specific recurrent layer for each task, \emph{R} stands for shared recurrent layer, and \emph{RF} stands for shared recurrent and feed-forward layer.}\label{sdp_LF_UF}
\end{figure}



==> fig/sdp_bert_id_ood.tex <==
\begin{figure}
\centering
\scalebox{0.5}{
\begin{tikzpicture}
\pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}

    \begin{groupplot}[group style = {group size = 2 by 2, horizontal sep = 30pt}, width = 4.0cm, height = 4.5.0cm]
    
%%%%%%%%%%%%%% in-domain LF  %%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ 
        title ={in-domain},
        width  = 0.55*\textwidth,
        height = 5cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=8pt,
        ylabel = {Labeled F1},
        %ylabel shift = 1 pt,
        ylabel near ticks,
        label style={font=\footnotesize},
        symbolic x coords={Single,SharedFNN,SharedFNN+SepRNN,SepFNN,SepFNN+SepRNN},
        xtick = data,
        scaled y ticks = false,
        ymin=55,
        legend cell align=left,
        legend style={at={(0.5,-1.6)},anchor=west,font=\scriptsize,column sep = 7pt, legend columns = 3},
    	point meta=explicit symbolic,
    	every node near coord/.append style={font=\footnotesize},
    	nodes near coords align={vertical},
    	title={in-domain}
    	]
    	
        \addplot[style={ggreen,fill=ggreen,mark=none}]
        	%no_bert
            coordinates {(Single,57.48) (SharedFNN,58.32) (SharedFNN+SepRNN,58.74) (SepFNN,59.29) (SepFNN+SepRNN,57.68)};
        \addlegendentry{\scriptsize{bo BERT}}%


        \addplot[style={bblue,fill=bblue,mark=none}]
        	%bert_source
            coordinates {(Single,58.2)
            (SharedFNN,58.98) (SharedFNN+SepRNN,58.53) (SepFNN,58.7) (SepFNN+SepRNN,58.45)};
        \addlegendentry{\scriptsize{Source BERT}}%


        \addplot[style={rred,fill=rred,mark=none}]
        	%bert_source_target
            coordinates {(Single,56.34)
            (SharedFNN,58.44) (SharedFNN+SepRNN,57.63) (SepFNN,58.33) (SepFNN+SepRNN,55.67)};
        \addlegendentry{\scriptsize{Source + Target BERT}}%


%%%%%%%%%%%%%% out-domain LF  %%%%%%%%%%%%%%%%%%%%
            
        \nextgroupplot[ 
        title={out-of-domain},
        width  = 0.55*\textwidth,
        height = 5cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=9pt,
        %ylabel = {Labeled F1},
        %ylabel shift = 1 pt,
        ylabel near ticks,
        label style={font=\footnotesize},
        symbolic x coords={Single,SharedFNN,SharedFNN+SepRNN,SepFNN,SepFNN+SepRNN},
        xtick = data,
        scaled y ticks = false,
        ymin=55,
    	point meta=explicit symbolic,
    	every node near coord/.append style={font=\footnotesize},
    	nodes near coords align={vertical},
    	]
    
        \addplot[style={ggreen,fill=ggreen,mark=none}]
        	%no_bert
            coordinates {(Single,58.75)
            (SharedFNN,60.5) (SharedFNN+SepRNN,60.81) (SepFNN,61.24) (SepFNN+SepRNN,59.83)};


        \addplot[style={bblue,fill=bblue,mark=none}]
        	%bert_source
            coordinates {(Single,60.01)
            (SharedFNN,61.08) (SharedFNN+SepRNN,60.85) (SepFNN,61.11) (SepFNN+SepRNN,60.84)}; 

        \addplot[style={rred,fill=rred,mark=none}]
        	%bert_source_target
            coordinates {(Single,57.88)
            (SharedFNN,60.38) (SharedFNN+SepRNN,59.87) (SepFNN,60.56) (SepFNN+SepRNN,58.19)};

%%%%%%%%%%%%%% in-domain UF  %%%%%%%%%%%%%%%%%%%%
        \nextgroupplot
        [
        width  = 0.55*\textwidth,
        height = 5cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=9pt,
        ylabel = {Unlbeled F1},
        ylabel near ticks,
        label style={font=\footnotesize},
        symbolic x coords={Single,SharedFNN,SharedFNN+SepRNN,SepFNN,SepFNN+SepRNN},
        xtick = data,
        scaled y ticks = false,
        ymin=72,
    	point meta=explicit symbolic,
    	every node near coord/.append style={font=\footnotesize},
    	nodes near coords align={vertical},
        ]
        
        \addplot[style={ggreen,fill=ggreen,mark=none}]
        	%no_bert
            coordinates {(Single,74.26)
            (SharedFNN,75.72) (SharedFNN+SepRNN,75.31) (SepFNN,76.43) (SepFNN+SepRNN,75.46)};
        
        \addplot[style={bblue,fill=bblue,mark=none}]
        	%bert_source
            coordinates {(Single,75.82)
            (SharedFNN,76.55) (SharedFNN+SepRNN,76.36) (SepFNN,76.8) (SepFNN+SepRNN,76.67)};   
        
        \addplot[style={rred,fill=rred,mark=none}]
        	%bert_source_target
            coordinates {(Single,74.97)
            (SharedFNN,77.05) (SharedFNN+SepRNN,76.44) (SepFNN,77.03) (SepFNN+SepRNN,75)};
        
%%%%%%%%%%%%%% out-domain UF  %%%%%%%%%%%%%%%%%%%%
    \nextgroupplot
        [
        width  = 0.55*\textwidth,
        height = 5cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=9pt,
        %ylabel = {Unlbeled F1},
        ylabel near ticks,
        label style={font=\scriptsize},
        symbolic x coords={Single,SharedFNN,SharedFNN+SepRNN,SepFNN,SepFNN+SepRNN},
        xtick = data,
        scaled y ticks = false,
        ymin=72,
        legend style = {
        column sep = 1pt, legend columns = 1,
        legend to name = bert_grouplegend,
        legend cell align={left}}
        ]
        
        \addplot[style={ggreen,fill=ggreen,mark=none}]
        	%no_bert
            coordinates {(Single,75.83)
            (SharedFNN,77.9) (SharedFNN+SepRNN,77.31) (SepFNN,78.15) (SepFNN+SepRNN,77.31)};
        
        \addlegendentry{\scriptsize{no BERT}}%

        
        \addplot[style={bblue,fill=bblue,mark=none}]
        	%bert_source
            coordinates {(Single,77.71)
            (SharedFNN,78.58) (SharedFNN+SepRNN,78.56) (SepFNN,79) (SepFNN+SepRNN,78.66)};
        \addlegendentry{\scriptsize{source BERT}}%

        
        \addplot[style={rred,fill=rred,mark=none}]
        	%bert_source_target
            coordinates {(Single,76.26)
            (SharedFNN,78.61) (SharedFNN+SepRNN,78.05) (SepFNN,78.64) (SepFNN+SepRNN,76.58)};
        \addlegendentry{\scriptsize{source & target BERT}}%

    \end{groupplot}
    
    %\node at ($(group c2r1) + (4.5,-5cm)$) {\ref{bert_grouplegend}}; 

\end{tikzpicture}
}
\caption[Performance of different MTL models after adding BERT features on the in-domain and out-of-domain test sets]{Labeled (top row) and unlabeled (bottom row) F1 scores for different MTL models after using BERT features. Graphs on the left and right columns show in-domain and out-of-domain results on the SemEval Czech test set respectively.}\label{sdp_bert_LF_UF}

\end{figure}



==> fig/sdp_network.tex <==
\begin{figure}[t!]
	\begin{center}
	\includegraphics[scale=0.45]{fig/sdp_network.pdf}     
	\end{center}
	\caption{Illustration of the supervised semantic dependency parsing system of \cite{dozat-manning-2018-simpler} that is used in this paper. We try different variants of layer sharing with a syntactic parser in order to leverage multitask learning.}\label{fig_sdp_supervised}
	
\end{figure}

==> fig/sdp_sepFNN.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{fig/sdp_mtl_sep.pdf}
        \caption{Shared BiLSTM.}
        \label{fig_sdp_mtl_sep}
    \end{subfigure}
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{fig/sdp_mtl_sep_sem.pdf}
        \caption{Task-specific BiLSM.}
        \label{fig_sdp_mtl_sep_sem}
    \end{subfigure}
    \caption[MTL model with task-specific FNN layer]{MTL models with task-specific FNN: (a) MTL model with a single BiLSTM shared across the tasks, (b) MTL model with a task-specific BiLSTM beside the shared BiLSTM}
    \label{fig_sdp_mtl_sharedFNN}
\end{figure*}

==> fig/srl_sdp.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{1\textwidth}

\centering
\begin{dependency}%[theme = simple]
	\begin{deptext}
		A \& similar \& technique  \& is \& almost \& impossible \& to \& apply \& to \& other \& crops\\
	\end{deptext}

\depedge[edge unit distance=1ex]{8}{3}{A1}
\depedge{8}{9}{A2}

\end{dependency}

\caption{Semantic dependencies in PropBank.}
\label{fig_propbank_srl}
\end{subfigure}


\begin{subfigure}[t]{1\textwidth}
	
	\centering
	\begin{dependency}%[theme = simple]
		\begin{deptext}
		A \& similar \& technique  \& is \& almost \& impossible \& to \& apply \& to \& other \& crops\\
		\end{deptext}
	
	\deproot{5}{TOP}
	\depedge{2}{3}{ARG1}
	\depedge{1}{3}{BV}
	\depedge{5}{6}{ARG1}
	\depedge{6}{8}{ARG1}
	\depedge[edge unit distance=1.5ex]{8}{3}{ARG2}
	\depedge[edge unit distance=1.7ex]{8}{11}{ARG3}
	\depedge{10}{11}{ARG1}
		
	\end{dependency}
	
	\caption{DELPH-IN Minimal Recursion Semantics–derived bi-lexical dependencies (DM)}
	\label{fig_DM_sdp}
\end{subfigure}

\caption[Bi-lexical semantic dependencies in PropBank compared to DM representation]{Bi-lexical semantic dependencies in (a) PropBank and (b) DM representation.}\label{fig_srl_sdp}

\end{figure*}

==> sdp_dd_results.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}

\pgfplotsset{small,samples=20,every tick label/.append style={font=\scriptsize}}

\begin{groupplot}[group style = {group size = 2 by 1, horizontal sep = 50pt}, width = 6.0cm, height = 5.0cm]
\nextgroupplot
[
width = 6.0cm,
height = 6cm,
xtick={0,1,2,3,4,5,6,7},
ylabel = {LF},
xlabel = {iteration},
ymax = 58,
axis lines=left,
grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10},
legend style = {
	column sep = 1pt,
	legend columns = 1,
	legend to name = grouplegend,
	legend cell align={left}},
	axis lines=left,
]

		\addplot[
		color=red,
		mark=triangle,
		]
		coordinates {
			(0,44.4)(1,52.8) (2,55.1) (3,55.4) (4,55.7) (5,55.9) (6,56.3) (7,56.1) 
		};\addlegendentry{\scriptsize{Density-driven}}
		
		
		
		\addplot[
		color=black,
		dashed,
		thick,
		]
		coordinates {
			(0,55.21) (1,55.21) (2,55.21) (3,55.21) (4,55.21) (5,55.21) (6,55.21) (7,55.21)
		}; \addlegendentry{\scriptsize{Single}}
		

		\addplot[
		color=green,
		dashed,
		thick,
		]
		coordinates {
			(0,57.09) (1,57.09) (2,57.09) (3,57.09) (4,57.09) (5,57.09) (6,57.09) (7,57.09)
		}; \addlegendentry{\scriptsize{MTL}}
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\nextgroupplot[
	width = 6.0cm,
	height = 6cm,
	xtick={0,1,2,3,4,5,6,7},
	ylabel = {\footnotesize{UF}},
	xlabel = {iteration},
	ymax = 78,
	axis lines=left,
	grid=both,grid style={line width=.1pt, draw=gray!10},major grid style={line width=.1pt,draw=gray!10},
	legend style = {
		column sep = 1pt,
		legend columns = 1,
		legend to name = grouplegend,
		legend cell align={left}},
	axis lines=left,
	]
	
	
	\addplot[
	color=red,
	mark=triangle,
	]
	coordinates {
		(0,61.9)(1,72.8) (2,73.6) (3,74.4) (4,74.3) (5,74.6) (6,74.3) (7,74.4)
	};\addlegendentry{\scriptsize{Density-driven}}%
	
	\addplot[
	color=black,
	dashed,
	thick,
	]
	coordinates {
		(0,74.06) (1,74.06) (2,74.06) (3,74.06) (4,74.06) (5,74.06) (6,74.06) (7,74.06)
	}; \addlegendentry{\scriptsize{Single}}%


	\addplot[
	color=green,
	dashed,
	thick,
	]
	coordinates {
		(0,76.59) (1,76.59) (2,76.59) (3,76.59) (4,76.59) (5,76.59) (6,76.59) (7,76.59)
	};\addlegendentry{\scriptsize{MTL}}%
	

	\end{groupplot}
	\node at ($(group c2r1) + (4.3,-1.4cm)$) {\ref{grouplegend}}; 
		
\end{tikzpicture}
\caption[Density-driven training of Czech SDP model]{Labeled (left) and unlabeled (right) F1-scores of our density-driven approach for different iterations. Dashed lines show results of the \emph{Single} and \emph{MTL} (TS.FNN) models trained on the entire projection data with and without multitasking respectively. All evaluations are performed on the SemEval 2015 Czech development data.}\label{sdp_dds_results}
\end{figure*}

==> sdp_network.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[scale=0.7]{sdp_network.pdf}  
	\caption[Graphical depiction of our supervised SDP model]{Illustration of the supervised semantic dependency parsing system of \cite{dozat-manning-2018-simpler}.}\label{fig_sdp_supervised}
\end{figure*}

==> sdp_params.tex <==
\begin{table}[t!]
\centering
\label{table:param}
\small
%\setlength{\tabcolsep}{2pt}
\begin{tabular}{ll}
\hline\hline
Hyperparameter & Size \\
\hline
Word embedding ($d_w$) & 100 \\
POS tag embedding ($d_{t}$) & 100 \\
BERT features ($d_{b}$) & 768 \\
LSTM hidden state ($d_h$) & 600 \\
LSTM hidden layer & 3 \\
FNN edge/label size & 600 \\
Word/POS dropout & 20\% \\
BiLSTM dropout & 25\% \\
FNN Edge dropout & 25\% \\ 
FNN Label dropout & 33\% \\
Inter. coef. ($\lambda$) &  0.025 \\
MTL Interpolation coef. ($\omega$) &  0.975 \\
Learning rate (Adam) & $0.001$ \\
Minibatch & $\sim$1K tok. \\
\hline\hline

\end{tabular}
\caption{Our SDP model parameters}\label{table:sdp_params}
\end{table}

==> sdp_sepFNN.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{sdp_mtl_sep.pdf}
        \caption{Shared BiLSTM.}
        \label{fig_sdp_mtl_sep}
    \end{subfigure}
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{sdp_mtl_sep_sem.pdf}
        \caption{Task-specific BiLSM.}
        \label{fig_sdp_mtl_sep_sem}
    \end{subfigure}
    \caption[MTL model with task-specific FNN layer]{MTL models with task-specific FNN: (a) The MTL model with one BiLSTM shared across tasks. (b) The MTL model with a task-specific BiLSTM in addition to the shared BiLSTM.}
    \label{fig_sdp_mtl_sharedFNN}
\end{figure}

==> sdp_sharedFNN.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.52\textwidth}
        \includegraphics[width=\textwidth]{sdp_mtl_shared.pdf}
        \caption{Shared BiLSTM.}
        \label{fig_sdp_mtl_shared}
    \end{subfigure}
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{sdp_mtl_shared_sem.pdf}
        \caption{Task-specific BiLSM.}
        \label{fig_sdp_mtl_shared_sem}
    \end{subfigure}
    \caption[MTL model with shared FNN layer]{MTL models with shared FNN: (a) The MTL model with one BiLSTM shared across tasks. (b) The MTL model with a task-specific BiLSTM in addition to the shared BiLSTM.}
    \label{fig_sdp_mtl_sharedFNN}
\end{figure}

==> supervised.tex <==
\section{Supervised Semantic Dependency Parsing\label{sec:sdp:super}}
The supervised semantic dependency parser used in our cross-lingual model is similar to the system introduces in \citep{dozat-manning-2018-simpler}. In order to make the original model scalable to our computational resources, we performed modifications in the input representation and parameters used in the model. Preliminary experiments confirmed equivalent performance on the development data to the original model. Following we describe the supervised SDP model used in our experiments with details.

Given a sentence $s = [s_i]_{i=1}^{n}$ with $n$ tokens, we represent each token $s_i$ with the vector $x_i$ by concatenating its word ($x^{we} \in \mathbb{R}^{d_w}$) and POS tag ($x^{te} \in \mathbb{R}^{d_t}$) embeddings:

\[
x_{i} =  [x_i^{we}; x_i^{te}]~~~\forall i \in [1,\cdots,n]
\]
$x_i^{we}$ itself is computed by summing over the following emebdding vectors:
\[
x_i^{we} = x_i^{re} + x_i^{pe} + x_i^{ce}
\]
where:
\begin{itemize}
	\item $x_i^{re} \in \mathbb{R}^{d_w}$ is a randomly initialized word embedding vector;
	\item $x_i^{pe} \in \mathbb{R}^{d_w} $ is a fixed external pre-trained 
	word embedding vector;
	\item $x_i^{char} \in \mathbb{R}^{d_w}$ is character level representation of each token $s_i$ and is obtained by running a one-layer BiLSTM on top of $s_i$ characters.
\end{itemize}
The recurrent representation of each token in $s$ is obtained by running a deep three-layered BiLSTM on top of the sentence tokens. We represent hidden representation of $s_i$ with $h_i$ which is the last hidden state of the deep BiLSTM for $s_i$:
\[
h_{i} = {\tt BiLSTM}(s_{1:n}; i) \in \mathbb{R}^{d_h}
\]
The hidden representation of each token ($h_i$) is then factorized into four vectors by feeding $h_i$ into four distinctly parameterized feed-forward neural networks:
\[
h_i^{(e,d)} = {\tt FNN}^{(e,d)}(h_i)~~~~ \forall e \in \{edge, label\};d \in \{dep, head\}
\]
The factorized hidden vectors are then used to compute bilinear scores for the edges and labels separately:
\[
score^{(e)}_{i,j}=  h_i^{T~(e,dep)} W^{e}  h_j^{(e,head)} ~~~~~~~ \forall e \in \{edge, label\}
\]
To decide if there is an edge between $s_i$ and $s_j$, the unlabeled parser uses a sigmoid function that simply labels $s_j$ as the head of $s_i$ if $score^{(edge)}_{i,j} \ge 0$. Given an edge between $s_i$ and $s_j$, the probability of having a certain label for the edge is then computed using:
\[
p(label|(i,j)) = {\tt Softmax_{label}(score^{(label)}_{i,j})}
\]  
The model is trained by back-propagating the linear interpolation of the edge and label loss values computed as:
\[
loss=\lambda loss^{label} + (1-\lambda)loss^{edge}  
\]
Figure \ref{fig_sdp_supervised} gives the graphical depiction of the supervised system we just described. Moreover, we use word dropout for dropping word and POS tag embeddings (independently) from the input layer. We further utilize dropout in the main BiLSTM network as well as edge/label FNN models.   


\input{fig/sdp_network.tex}




==> tables/results_od.tex <==
\begin{table*}[t!]
    \centering
    %\scriptsize
     %\renewcommand{\arraystretch}{0.75}
     %\setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|c c | c | c c | c c | c c || c c }
    \hline\hline
      \multirow{2}{*}{Model} & \multicolumn{2}{c}{Shared} &  Task & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{+ ELMO}  & \multicolumn{2}{c}{+ mBERT}  & \multicolumn{2}{c}{Supervised} \\ 
      
 &  RNN & FNN & RNN &  LF & UF & LF & UF & LF & UF & LF & UF \\ \hline\hline
Single &  & &  &  58.8 & 75.8 & 59.0 & 75.8 &  57.9 & 76.3  & 70.4 & 86.8 \\ 
Multitask  & \checkmark & \checkmark &   & 60.5 & 77.9 & 61.4 & 78.5  & 60.4 & {\bf 78.6}  & 70.8 & 87.3 \\ 
Multitask   & \checkmark  & &  &  61.2 & 78.2 & {\bf 61.5} & 78.2  &  60.6 & {\bf 78.6}    & 70.8 & 87.0 \\ 
Multitask   & \checkmark  & & \checkmark   &  59.9 & 77.1 & 61.4 & 77.5  &  58.2 & 76.6   & 69.7 & 86.4 \\ 
Multitask  & \checkmark  & \checkmark  & \checkmark  & 60.8 & 77.3 & 60.6 & 77.5  &  59.9 & 78.1   & 71.1 & 87.3 \\\hline
    \end{tabular}
    \caption{F1 Results on the out-of-domain Czech test data in different settings. The base model does not use contextualized word embeddings. \emph{Task RNN} refers to an extra task-specific embedding in the multitask setting.  In all multitask settings, the embedding layers are shared across tasks.}
    \label{tab:ood_results}
\end{table*}
